MalAlgoQA: Pedagogical Evaluation of Counterfactual Reasoning in Large Language Models and Implications for AI in Education

This paper introduces MalAlgoQA, a novel dataset designed to evaluate the counterfactual reasoning capabilities of Large Language Models (LLMs) through a pedagogical approach. The dataset comprises mathematics and reading comprehension questions, each accompanied by four answer choices and their corresponding rationales. At the heart of MalAlgoQA are ``malgorithms'' - rationales behind incorrect answer choices that represent flawed yet logically coherent reasoning paths. These malgorithms serve as counterfactual scenarios, allowing us to assess an LLM's ability to identify and analyze flawed reasoning patterns. We propose the Malgorithm Identification task, where LLMs are assessed based on their ability to identify corresponding malgorithm given an incorrect answer choice. To evaluate the model performance, we introduce two metrics: Algorithm Identification Accuracy (AIA) for correct answer rationale identification, and Malgorithm Identification Accuracy (MIA) for incorrect answer rationale identification. Our experiments reveal that state-of-the-art LLMs exhibit significant performance drops in MIA compared to AIA, highlighting the challenges in counterfactual reasoning. Surprisingly, we find that the chain-of-thought prompting technique not only fails to consistently enhance MIA but can sometimes lead to underperformance compared to simple prompting. These findings have important implications for developing LLMs with improved counterfactual reasoning, particularly relevant for AI-powered tutoring systems, where identifying and addressing student misconceptions is essential. MalAlgoQA dataset is available \href{https://github.com/luffycodes/MalAlgoQA-Dataset}{here}.

==> sections/experiments_questions.tex <==
\subsection{Experimental Setting}
\begin{itemize}
% \item How do the LLMs perform in the Cause Identification, Effect Identification, and Control tasks?
% \item Are there significant differences in performance between the three tasks?
\item How does the performance compare between zero-shot and few-shot learning settings?
\item What is the impact of chain-of-thought prompting on LLM performance in each task?
\end{itemize}

\subsection{Model Comparison}
\subsubsection{Overall Performance}
\begin{itemize}
    \item How do the three models compare in terms of overall accuracy on the MalAlgoQA dataset?
    \item Are there significant differences in performance between the models?
    \item Which model performs the best overall, and by what margin?
\end{itemize}

\subsubsection{Performance Across Grade Levels}
\begin{itemize}
    \item How does the performance of each model vary across different grade levels?
    \item Are there specific grade levels where one model outperforms the others?
    \item Is the relative performance of the models consistent across grade levels?
\end{itemize}

\subsubsection{Performance Across Content Classifications}
\paragraph{Mathematics}
\begin{itemize}
    \item How does the performance of each model vary across different mathematics content classifications?
    \item Are there specific content areas where one model excels compared to the others?
\end{itemize}

\paragraph{Reading Comprehension}
\begin{itemize}
    \item How does the performance of each model vary across different reading comprehension content classifications?
    \item Is there a significant difference in the relative performance of the models between the two content classifications?
\end{itemize}

\subsubsection{Performance Across DOK Levels}
\begin{itemize}
    \item How does the performance of each model vary across different DOK levels?
    \item Are there specific DOK levels where one model outperforms the others?
    \item Is the relative performance of the models consistent across DOK levels?
\end{itemize}

\subsubsection{Impact of Question and Rationale Characteristics}
\begin{itemize}
    \item Does the impact of question length on performance differ between the models?
    \item Is the correlation between the length of answer rationales and performance consistent across the models?
\end{itemize}

\subsection{Comparison of Few-Shot Learning Approaches}
\begin{itemize}
    \item How does the performance of LLMs compare between zero-shot and few-shot learning settings?
    \item Does the number of few-shot examples impact LLM performance?
    \item Are there specific grade levels, content classifications, or DOK levels where few-shot learning significantly improves LLM performance?
\end{itemize}

\subsection{Impact of Chain-of-Thought Prompting}
\begin{itemize}
    \item How does the performance of LLMs compare between standard prompting and chain-of-thought prompting?
    \item Does chain-of-thought prompting improve LLM performance across different grade levels, content classifications, and DOK levels?
    \item Are there specific question types or characteristics where chain-of-thought prompting is particularly effective?
\end{itemize}

\subsection{Error Analysis}
\begin{itemize}
    \item What are the common types of errors made by LLMs?
    \item Are there specific question types or characteristics that consistently challenge LLMs?
    \item How do the error patterns differ between mathematics and reading comprehension questions?
    \item Can the error analysis provide insights into the reasoning capabilities and limitations of LLMs?
\end{itemize}

This template prioritizes the comparison of the three models across various dimensions, followed by the analysis of few-shot learning approaches and the impact of chain-of-thought prompting. The error analysis section is placed last, as it provides insights into the limitations and potential areas for improvement in LLM performance.

==> tables/math_full_malagoqa.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{cccccc}
\toprule
\textbf{LLM} & \textbf{Num Shots} & \textbf{Prompting} & \textbf{MCQ} & \textbf{AIA} & \textbf{MIA} \\
\midrule
GPT 4o  & 0 & Simple & 90.11 & 92.06 & 62.82 \\
GPT 4o  & 5 & Simple &  & 90.61 & 64.99 \\
GPT 4o  & 0 & CoT & 97.61 & 95.65 & 66.1 \\
GPT 4o  & 5 & CoT &  & 95.49 & 65.1 \\
\midrule
LLaMA-70B  & 0 & Simple & 73.83 & 94.31 & 50.22 \\
LLaMA-70B  & 5 & Simple &  & 93.65 & 48.31 \\
LLaMA-70B  & 0 & CoT & 90.72 & 95.47 & 55.32 \\
LLaMA-70B  & 5 & CoT &  & 95.89 & 50.6 \\
\hline
GPT 3.5  & 0 & Simple & 52.85 & 77.08 & 35.8 \\
GPT 3.5  & 5 & Simple &  & 76.85 & 34.61 \\
GPT 3.5  & 0 & CoT & 82.53 & 86.28 & 14.74 \\
GPT 3.5  & 5 & CoT &  & 81.87 & 17.06 \\
\midrule
LLaMA-8B  & 0 & Simple & 45.79 & 75.29 & 34.81 \\
LLaMA-8B  & 5 & Simple &  & 80.32 & 38.41 \\
LLaMA-8B  & 0 & CoT & 70.68 & 83.07 & 27.05 \\
LLaMA-8B  & 5 & CoT &  & 83.05 & 31.39 \\
\bottomrule
\end{tabular}
\caption{Results for Math subject in the Cause Identification task.}
\label{tab:math_results}
\end{table*}

==> tables/read_full_malagloqa.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|cccccc|}
% \toprule
\hline
\textbf{LLM} & \textbf{Num Shots} & \textbf{Prompting} & \textbf{MCQ} & \textbf{AIA} & \textbf{MIA} \\
\hline
GPT 4o  & 0 & Simple & 95.86 & 98.23 & 82.8 \\
GPT 4o  & 0 & CoT & 95.52 & 97.88 & 68.63 \\
\hline
LLaMA-70B  & 0 & Simple & 89.45 & 95.72 & 60.0 \\
LLaMA-70B  & 0 & CoT & 89.27 & 94.6 & 58.4 \\
\hline
GPT 3.5  & 0 & Simple & 84.83 & 95.05 & 13.98 \\
GPT 3.5  & 0 & CoT & 81.66 & 85.82 & 8.61 \\
\hline
LLaMA-8B  & 0 & Simple & 73.96 & 89.62 & 19.89 \\
LLaMA-8B  & 0 & CoT & 78.05 & 89.52 & 15.47 \\
\hline
% \bottomrule
\end{tabular}
\caption{Results for Reading subject in the Cause Identification task.}
\label{tab:reading_results}
\end{table*}

==> tables/simple_vs_cot.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|ccccc|}
\toprule
\textbf{LLM} & \textbf{Subject} & \textbf{Prompting} & \textbf{AIA} & \textbf{MIA} \\
\hline
GPT-4o & Math & CoT & 95.49 & 65.10 \\
       &      & Simple & 90.61 & 64.99 \\
       & Reading & CoT & 97.88 & 68.63 \\
       &      & Simple & 98.23 & 82.80 \\
\hline
LLaMA-70B & Math & CoT & 95.89 &	50.6 \\
          &      & Simple & 93.65	& 48.31 \\
          & Reading & CoT & 94.6 &	58.4 \\
          &      & Simple & 95.72	& 60.0 \\
\hline
\end{tabular}
\caption{Algorithm Identification Accuracy (AIA) and Malgorithm Identification Accuracy (MIA) for Math and Reading subjects in zero-shot setting.}
\label{tab:aia_mia}
\end{table*}
